GL(2)-structures of the Langlands global program

All kinds of global correspondences of Langlands are evaluated from the functional representation spaces of the algebraic bilinear semigroups GL2(.x.) with entries in products,right by left,of sets of archimedean increasing completions. Degenerate singularities on these functional representation spaces can give rise,by versal deformations and blowups of these,to one or two new covering functional representation spaces of GL2(.x.) according to the type of considered singularities. The discovered correspondences of Langlands are associated with singular and nonsingular universal GL(2)-structures.

==> GL2-2.tex <==
\section{Dark energy structure of elementary particles}

\subsection{Nature of algebraic quantum theory}

The {\bf algebraic quantum theory is a theory of internal structure of elementary particles\/}: this internal structure {\bbf is a universal mathematical structure in the heart of the global program of Langlands\/} developed by the author in \cite{Pie3}, \cite{Pie4}, and {\bbf resulting from one-to-one correspondences between representations of Galois groups and their holomorphic representations (and cuspidal forms) affected by singularities\/}.
\vskip 11pt

A QT is thus a new quantum field theory \cite{F-R-S} based on algebraic geometry and number theory and not deduced from classical mechanics as QFT but reaching the same objectives as QFT and even more.
\vskip 11pt

\subsection{Quantization by means of algebraic quanta of structure}

Indeed, {\bbf AQT is a structural algebraic quantum field theory whose spatial building blocks are space structure algebraic quanta defined as irreducible closed algebraic subsets of degree $N$\/}.

Remark that the energy quanta are shifted spatial algebraic quanta resulting from differential Galois theory generating Galois groupoids on manifolds as described in \cite{Pie5}.
\vskip 11pt

Assume that these structure algebraic quanta have a universal representation space given by open balls of radii equivalent to the Planck constant $\hbar $ in the sense that all the roots of the splitting field of an algebraic quantum are mapped in an open ball of radius of magnitude of $\hbar$.

{\bbf These algebraic quanta can then be considered as big points at the Planck scale\/}.
\vskip 11pt

{\bbf By a change of scale \cite{Pie2}, each algebraic quantum, i.e. a quantum big point, can correspond to a macroscopic point of classical mechanics or general relativity\/} if all points of this algebraic quantum implode on the considered open ball center viewed as the corresponding macroscopic point.  This implosion of all points of an algebraic quantum inside an open ball of magnitude $\hbar$ can be described mathematically by {\bbf a projective map $P_{ac}$ from all roots of the algebraic quantum onto the center of the considered open ball\/}.

This projective map is associated with a metric (tensor) contraction if the considered closed algebraic subset of the algebraic quantum is compact.

It {\bbf describes the transition from the quantum level to the classical level in the frame of algebraic geometry\/} taking into account that a set of $q$ neighbouring algebraic quanta imploding onto their centers gives rise to a continuum compact subset of $q$ ``classical'' points.
\vskip 11pt

{\bbf This projective map $P_{ac}$ is the inverse analogue of the deformation quantization\/} \cite{F-L-S} consisting in deforming the algebra $A$ of classical observables over a ground field $k$ into the algebra $\wt A$ over $k[[\hbar]]$ in such  way that $\wt A/\hbar \wt A\approx A$ where $\wt A$ is  topologically free $k[[\hbar]]$-module.  This leads to the existence of a new product $u\star v$, for $u,v\in A$, expanded in formal series:
\[ u\star v=u \ v+\sum_{r=1}^\infty \hbar^r\ c_r(u,v)\]
where $c_r$ is a Hochschild $2$-cochain \cite{Ster}, \cite{Ger}.
\vskip 11pt

\subsection{Fusion of quantum mechanics with special relativity by bisemistructures}

{\bbf The fusion of quantum mechanics with special relativity is still an open problem\/} since ``no exactly solved nontrivial model of interacting quantum field theory on Minkowsky space is yet known'' as noticed by S. Doplicher in \cite{Dop}.

{\bbf This question was envisaged in AQT as a crucial step by considering a completely bilinear version of QFT by means of bisemistructures\/} introduced by the author in \cite{Pie6}.
\vskip 11pt

{\bbf A fundamental bisemistructure refers to a bisemigroup appearing in the triple\linebreak $(G_L,G_R,G\RL)$\/} where:
\Bean
\item $GL$ \resp{$G_R$} is a \lr semigroup under the addition of its \lr elements $g_{L_i}$ \resp{$g_{R_i}$} restricted to (or referring to) the upper \resp{lower} half space.

\item $G\RL$ is a bilinear semigroup whose bielements $(g_{R_i}\times g_{L_i})$ are submitted to the cross binary operation according to:
\begin{eqnarray*}
 G\RL\u\times G\RL&\To&G\RL\;,\\
 (g_{R_i}\times (g_{L_i})\u\times (g_{R_j}\times (g_{L_j})&\To & 
 (g_{R_i}+ g_{R_j})\times (g_{L_i}+ g_{L_j})\;,
 \end{eqnarray*}
 leading to cross products $(g_{R_i}\times g_{L_i})$ and $ (g_{R_j}\times g_{L_j})$.
 \Ee
 \vskip 11pt
 
 Important bisemigroups are {\bbf algebraic bilinear semigroups of matrices $\GL_2(\wt F_R\times \wt F_L)$ interpreted as (bilinear) representations of product, right by left, of global Weil (or Galois) groups in the frame of the global program of Langlands \cite{Pie3} and leading to a consistent algebraic definition of  elementary particle quantum fields having a bilinear character and inducing a ``bi-semi'' particle structure as outlined in section~2.6\/}.
 
 An algebraic bilinear semigroup $\GL_2(\wt F_R\times \wt F_L)$ then decomposes according to:
 \[ \GL_2(\wt F_R\times \wt F_L)=T^t_2(\wt F_R)\times T_2(\wt F_L)\]
 where $T^t_2(\wt F_R)$ \resp{$T_2(\wt  F_L)$} is a right \resp{left} linear semigroup of lower \resp{upper} triangular matrices with entries in $\wt F_R$
 \resp{$\wt F_L$} which are right \resp{left} algebraic symmetric extensions of a global number field of characteristic $0$.
 \vskip 11pt
 
 Let $L_{\o v}=\{L_{\o v_{\mu ,m_\mu }}\}_{\mu ,m_\mu }$
\resp{$l_{v}=\{L_{ v_{\mu ,m_\mu }}\}_{\mu ,m_\mu }$}
denote the set of right \resp{left} real pseudoramified completions associated with $\wt F_R$ \resp{$\wt F_L$} and characterized by degrees
\[
[L_{\o v_{\mu ,m_\mu }}:k]=\star +\mu \cdot N\;,
\rresp{[L_{v_{\mu ,m_\mu }}:k]=\star +\mu \cdot N}\]
which are integers modulo $N$, where $\star$ is an integer inferior to $N$.

Let $M_R(L_{\o v})\otimes M_L(L_v)$ be the representation space $\Repsp(\GL_2(L_{\o v}\times L_v))$ of the bilinear algebraic semigroup
$\GL_2(L_{\o v}\times L_v)$ over products of pairs of real completions.

It decomposes into a set of conjugacy class representatives on the real pseudoramified completions 
$L_{\o v_{\mu ,m_\mu }}$ and
$L_{v_{\mu ,m_\mu }}$ according to \cite{Pie7}:
\[ M_R(L_{\o v})\otimes M_L(L_v)=\{M_{\o v_{\mu ,m_\mu }}\otimes
M_{v_{\mu ,m_\mu }}\}_{v_{\mu ,m_\mu }}\]
where $m_\mu $ labels the multiplicity of the $\mu $-th conjugacy class representative
$M_{\o v_{\mu ,m_\mu }}\otimes M_{v_{\mu ,m_\mu }}$.
\vskip 11pt

Let $\phi _R(M_{\o v_{\mu ,m_\mu }})$
\resp{$\phi _L(M_{v_{\mu ,m_\mu }})$} be a complex-valued differentiable function over the\linebreak
$(\mu ,m_\mu )$-th conjugacy class representative of
$T^t_2(L_{\o v})$
\resp{$T_2(L_{v})$} and let
$\phi _R(M_{\o v_{\mu ,m_\mu }})\otimes \phi _L(M_{v_{\mu ,m_\mu }})$ denote the corresponding bifunction on $M_{\o v_{\mu ,m_\mu }}\otimes M_{v_{\mu ,m_\mu }}$.

Then, the set $\{\phi _R(M_{\o v_{\mu ,m_\mu }})\}_{\mu ,m_\mu }$
\resp{$\{\phi _L(M_{v_{\mu ,m_\mu }})\}_{\mu ,m_\mu }$}
of $\cit$-valued differentiable functions, localized in the lower \resp{upper} half space is the set
$\Gamma (\phi _R(M_R(L_{\o v})))$
\resp{$\Gamma (\phi _L(M_L(L_{v})))$}
 of right \resp{left} sections of the semisheaf of rings 
 $\phi _R(M_R(L_{\o v}))$
\resp{$\phi _L(M_L(L_{v}))$}.

And, {\bbf the set 
$\{\phi _R(M_{\o v_{\mu ,m_\mu }})\otimes \phi _L(M_{v_{\mu ,m_\mu }})\}_{\mu ,m_\mu }$
of differentiable bifunctions constitutes the set
$\Gamma (\phi _R(M_R(L_{\o v}))\otimes \phi _L(M_L(L_{v})))$ of bisections of the bisemisheaf of rings
$\phi _R(M_R(L_{\o v})\otimes \phi _L(M_L(L_{v})$
over $\GL_2(L_{\o v}\times L_v)$\/}.
\vskip 11pt

\subsection{Proposition}

{\bbf\em The bisemisheaf of rings $\phi _R(M_R(L_{\o v})\otimes \phi _L(M_L(L_{v})$ is a physical bosonic quantum string field of an elementary particle\/}.
\vskip 11pt

\begin{proof} Let $L^T_{\o v}=\{L^T_{\o v_{\mu ,m_\mu }}\}_{\mu ,m_\mu }$
\resp{$L^T_{v}=\{L^T_{v_{\mu ,m_\mu }}\}_{\mu ,m_\mu }$} be the set  of \rl real pseudoramified {\bf toroidal completions\/} obtained from $L_{\o v}$ \resp{$L_v$} by a toroidal compactification of the corresponding completions
$L_{\o v_{\mu ,m_\mu }}$
\resp{$L_{v_{\mu ,m_\mu }}$} \cite{Pie3}.

The set $\{L^T_{\o v_{\mu ,m_\mu }}\}_{m_\mu }$
\resp{$\{L^T_{v_{\mu ,m_\mu }}\}_{m_\mu }$}
of $\mu $-th completions are then semicircles covering a $2$-dimensional \rl semitorus $T^2_R(\mu )$ \resp{$T^2_L(\mu )$}, localized in the lower \resp{upper} half space.
\vskip 11pt

Assume that the degree of $L^T_{\o v_{\mu ,m_\mu }}$ and of
$L^T_{v_{\mu ,m_\mu }}$ is given by
\[[L^T_{\o v_{\mu ,m_\mu }}]\equiv [L^T_{v_{\mu ,m_\mu }}]=\mu \ N\;.\]
Then, $L^T_{\o v_{\mu ,m_\mu }}$
and $L^T_{v_{\mu ,m_\mu }}$ are toroidal completions or semicircles at $\mu $ quanta, a quantum being an irreducible completion of degree $N$.
\vskip 11pt

As we are essentially interested in circles, toroidal completions
$L^T_{\o v_{2\mu ,m_{2\mu }}}$
and $L^T_{v_{2\mu ,m_{2\mu} }}$ characterized by degrees:
\[[L^T_{\o v_{2\mu ,m_{2\mu} }}]\equiv [L^T_{v_{2\mu ,m_{2\mu} }}]=2\ \mu \ N\]
will be taken into account.

By this way, the corresponding completions $L_{\o v_{2\mu ,m_{2\mu }}}$
and $L_{v_{2\mu ,m_{2\mu} }}$ are closed paths or closed strings.
\vskip 11pt

{\bbf Now, each product
$\{L^T_{\o v_{2\mu ,m_{2\mu }}}\otimes L^T_{v_{2\mu ,m_{2\mu} }}\}$ of symmetric circles\/} rotating in opposite senses according to \cite{Pie2} {\bbf is the representation of an harmonic oscillator\/}.  This is also the case for the product $\{L_{\o v_{2\mu ,m_{2\mu }}}\otimes L_{v_{2\mu ,m_{2\mu} }}\}$ of corresponding completions homeomorphic to
$\{L^T_{\o v_{2\mu ,m_{2\mu }}}\otimes L^T_{v_{2\mu ,m_{2\mu} }}\}$ and for the product
$\{\phi _R(M_{\o v_{2\mu ,m_{2\mu }}})\otimes \phi _L(M_{v_{2\mu ,m_{2\mu} }})\}$ of $\cit$-valued differentiable functions.
\vskip 11pt

Consequently, {\bbf the set of packets
$\{\phi _R(M_{\o v_{2\mu ,m_{2\mu }}})\otimes \phi _L(M_{v_{2\mu ,m_{2\mu} }})\}_{2\mu ,m_{2\mu }}$ of bifunctions\/} on
$\{L{\o v_{2\mu ,m_{2\mu }}}\otimes L_{v_{2\mu ,m_{2\mu} }}\}_{2\mu ,m_{2\mu }}$ {\bbf behaves like a set of packets of harmonic oscillators characterized by increasing integers $2\mu $\/}.

Thus, the bisemisheaf of rings
\[\phi _R(M_R(L_{\o v}))\otimes \phi _L(M_L(L_{v}))=
\{\phi _R(M_{\o v_{2\mu ,m_{2\mu }}})\otimes \phi _L(M_{v_{2\mu ,m_{2\mu} }})\}_{2\mu ,m_{2\mu }}\] is a physical string field.
\vskip 11pt

{\bbf It is a quantum string field because the set of sections of the bisemisheaf
$\phi _R(M_R(L_{\o v}))\linebreak\otimes \phi _L(M_L(L_{v}))$ is a tower of increasing bistrings\/}, i.e. products of symmetric right and left strings,  behaving like harmonic oscillators and characterized by a number of increasing biquanta, $2\mu \le\infty $, corresponding to the normal modes of the string field.

{\bbf This quantum string field is a bosonic field\/} because biquanta can be added to (i.e. created) or removed (i.e. annihilated) from these bistrings by Galois automorphisms or antiautomorphisms as developed in \cite{Pie1} and because each bistring with degree $2\mu $ was interpreted as a ``bound bisemiphoton'' at $2\mu $ biquanta.
\end{proof}
\vskip 11pt

\subsection{Corner-Stone of the unification of GR with QFT: vacuum space-time substructure}

{\bbf The other great challenge of AFT is the unification of QFT with GR.  The corner-stone of this possible unification is the connection between the vacuum state of QFT and the cosmological constant of GR as recalled in section 1\/}.  This vacuum of QFT was assumed in \cite{Pie1} and in \cite{Pie2} to be of expanding space-time type in order to correspond to the de Sitter solution of the equations of GR and to be shared out amongst the own vacua of the elementary particles.  Under this hypothesis, {\bbf the vacuum substructure of every elementary particle must have an expanding space-time nature and can be described by a time and a space quantum string field.

The generative string field is the time string field considered as a reservoir of space having an inertial effect on the space string field localized in an orthogonal space\/}.
\vskip 11pt

To the time string field, noted in condensed notation $(\wt M^T_{ST_R}\otimes \wt M^T_{ST_L})$, corresponds {\bbf an operator-valued time string field
 $(\wt M^{T_p}_{ST_R}\otimes \wt M^{T_p}_{ST_L})$ obtained from
 $(\wt M^T_{ST_R}\otimes \wt M^T_{ST_L})$ by the action of the differential bioperator\/}:
\[ T_{R;ST}\otimes T_{L;ST}: \qquad 
 (\wt M^T_{ST_R}\otimes \wt M^T_{ST_L}) \To
 (\wt M^{T_p}_{ST_R}\otimes \wt M^{T_p}_{ST_L})\]
 in such a way that
 \[ T_{R;ST}\otimes T_{L;ST}=
\L(-i\F{\hbar_{ST}}{c_{t\to r;ST}}\overrightarrow s_{0_R}\ \frac \partial{\partial t_0}\R)\otimes
\L( i\F{\hbar_{ST}}{c_{t\to r;ST}}\overrightarrow s_{0_L}\ \frac \partial{\partial t_0}\R)\]
acts on each bisection or bistring
\[ \phi _{\mu _R}\otimes \phi _{\mu _L}\equiv 
\phi _R(M_{\o v_{2\mu ,m_{2\mu }}})\otimes
\phi _L(M_{v_{2\mu ,m_{2\mu }}})\]
where $\hbar_{ST}$ and $c_{t\to r}$ are respectively the Planck constant and the velocity of light at this (space-)time internal level, i.e. the level of the dark energy.

$T_{R;ST}$ and
$T_{L;ST}$ are directional derivatives in the time variable $t_0$ in the directions 
$\overrightarrow s_{0_R}$ and
$\overrightarrow s_{0_L}$ respectively.

As each left string rotates in opposite sense with respect to the corresponding symmetric right string and has two senses of rotation, it corresponds to the time string field 
$(\wt M^{T_p}_{ST_R}\otimes \wt M^{T_p}_{ST_L})$ of spin $1/2$.
\vskip 11pt

The operator-valued {\bbf space string field, noted
$(\wt M^{S_p}_{ST_R}\otimes \wt M^{S_p}_{ST_L})$, can be generated from the (operator-valued) time string field
$(\wt M^{T_p}_{ST_R}\otimes \wt M^{T_p}_{ST_L})$ by the (composition of) morphisms of its right and left semifields\/}:
\begin{align*}
\gamma _{t\to r} \circ E_R : \quad \wt M^{T_p}_{ST_R}&\To \wt M^{T_p(r)}_{ST_R}\oplus \wt M^{S_p}_{ST_R})\\
\rresp{\gamma _{t\to r} \circ E_L : \quad \wt M^{T_p}_{ST_L}&\To \wt M^{T_p(r)}_{ST_L}\oplus \wt M^{S_p}_{ST_L})}
\end{align*}
where $E_R$ \resp{$E_L$} is an endomorphism \cite{Pie1} based on Galois antiautomorphisms and transforming the semifield 
$\wt M^{T_p}_{ST_R}$  \resp{$\wt M^{T_p}_{ST_L}$} into a disconnected time residue semifield 
$\wt M^{T_p(r)}_{ST_R}$  \resp{$\wt M^{T_p(r)}_{ST_L}$}
and into a complementary time semifield
$\wt M^{T_p(i)}_{ST_R}$ \resp{$\wt M^{T_p(i)}_{ST_L}$} which, projected through the origin into the orthogonal three-dimensional space by the morphism
$\gamma _{t\to r}$, gives rise to the space semifield
$\wt M^{S_p}_{ST_R}$ \resp{$\wt M^{S_p}_{ST_L}$}.
\vskip 11pt

{\bf The} (operator-valued) {\bf space-time fields
$(\wt M^{T_p(r)}_{ST_R}\oplus \wt M^{S_p}_{ST_R})\otimes
(\wt M^{T_p(r)}_{ST_L}\oplus \wt M^{S_p}_{ST_L})$ then describe the dynamics of the internal vacuum structure of a lepton of the first family\/}, i.e. essentially the electron and its neutrino $\nu _{e^-}$.  Referring to the introduction, {\bbf these space-time fields are responsible for the dark energy structure of the electron (and of its neutrino)\/}.

They decompose as a bisemistructure \cite{Pie6} into the following disconnected space-time (i.e. dark energy) subfields
\begin{multline*}
(\wt M^{T_p-S_p}_{ST_R}\otimes \wt M^{T_p-S_p}_{ST_L})\equiv
(\wt M^{T_p}_{ST_R}\oplus \wt M^{S_p}_{ST_R})\otimes
(\wt M^{T_p}_{ST_L}\oplus \wt M^{S_p}_{ST_L})\\
\To
(\wt M^{T_p-S_p}_{ST_R}\otimes_D \wt M^{T_p-S_p}_{ST_L})\oplus
(\wt M^{S_p}_{ST_R}\otimes_{\rm magn} \wt M^{S_p}_{ST_L})\oplus
(\wt M^{S_p(T_p)}_{ST_R}\otimes_{\rm elec} \wt M^{T_p(S_p)}_{ST_L})
\end{multline*}
where:
\Bean
\item $(\wt M^{T_p-S_p}_{ST_R}\otimes_D \wt M^{T_p-S_p}_{ST_L})$ is a four-dimensional bilinear diagonal subfield;

\item $(\wt M^{S_p}_{ST_R}\otimes_{\rm magn} \wt M^{S_p}_{ST_L})$ is a three-dimensional off-diagonal magnetic subfield generated from the exchange of magnetic biquanta between the right and left space subsemifields 
$\wt M^{S_p}_{ST_R}$ and $\wt M^{S_p}_{ST_L}$ as described in \cite{Pie7};

\item $\wt M^{S_p(T_p)}_{ST_R}\otimes_{\rm elec} \wt M^{T_p(S_p)}_{ST_L})$ is a three-dimensional off-diagonal electric subfield generated from the exchange of electric biquanta between the right space \resp{right time} and left time \resp{left space} subsemifields \cite{Pie1}.
\Ee
\vskip 11pt

{\bbf From a bigger time string field\/} (noted 
$\wt M^{(\rm Bar);T_p}_{ST_R}\otimes \wt M^{(\rm Bar);T_p}_{ST_L}$) {\bbf (i.e. a time baryonic string field\/} with much more packets of bistrings),
{\bbf another endomorphism $E_{t_R}$
\resp{$E_{t_L}$} can be envisaged\/} in such a way that
$E_{t_R}$
\resp{$E_{t_L}$} {\bbf participates in the decomposition of the \rl baryonic time semifield 
$\wt M^{(\rm Bar);T_p}_{ST_R}$ \resp{$\wt M^{(\rm Bar);T_p}_{ST_L}$}
into a residue time semifield
$\wt M^{(\rm Bar);T_p(r)}_{ST_R}$ \resp{$\wt M^{(\rm Bar);T_p(r)}_{ST_L}$} and into three connected complementary semiquark time semifields
$\{\wt M^{q_i;T_p}_{ST_R}\}_{i=1}^3$
\resp{$\{\wt M^{q_i;T_p}_{ST_L}\}_{i=1}^3$}} according to:
\begin{align*}
\gamma _{t\to \oplus t_i}\circ E_{t_R}: \quad
\wt M^{(\rm Bar);T_p}_{ST_R} &\To
\wt M^{(\rm Bar);T_p(r)}_{ST_R} \bigoplus_{i=1}^3 \wt M^{q_i;T_p}_{ST_R} \\
\rresp{
\gamma _{t\to \oplus t_i}\circ E_{t_L}: \quad
\wt M^{(\rm Bar);T_p}_{ST_L} &\To
\wt M^{(\rm Bar);T_p(r)}_{ST_L} \bigoplus_{i=1}^3 \wt M^{q_i;T_p}_{ST_L}}
\end{align*}
where:
\Bi
\item $E_{t_R}$
\resp{$E_{t_L}$} is the baryonic endomorphism based on Galois antiautomorphisms decomposing
$\wt M^{(\rm Bar);T_p}_{ST_R}$
\resp{$\wt M^{(\rm Bar);T_p}_{ST_L}$} into a core residue time semifield
$\wt M^{(\rm Bar);T_p(r)}_{ST_R}$
\resp{$\wt M^{(\rm Bar);T_p(r)}_{ST_L}$} and into a connected complementary time semifield 
$\wt M^{(\rm Bar);T_p(i)}_{ST_R}$
\resp{$\wt M^{(\rm Bar);T_p(i)}_{ST_L}$};
\item $\gamma _{t\to \oplus t_i}$ is the morphism sending
$\wt M^{(\rm Bar);T_p(i)}_{ST_R}$
\resp{$\wt M^{(\rm Bar);T_p(i)}_{ST_L}$} into a three-dimensional connected complementary time semispace and transforming it into the three time semifields
$\{\wt M^{q_i;T_p}_{ST_R}\}_{i=1}^3$
\resp{$\{\wt M^{q_i;T_p}_{ST_L}\}_{i=1}^3$} of the semiquarks.
\Ei

The time string semifields of the three right \resp{left} semiquarks are then connected to the residue core time semifield of the \rl semibaryon leading to the confinement of these.

The space semifield
$\wt M^{q_i;S_p}_{ST_R}$
\resp{$\wt M^{q_i;S_p}_{ST_L}$} of the three \rl semiquarks can be generated by
$(\gamma _{t_{i_R}\to r_{i_R}}\circ E_{i_R})$
\resp{$(\gamma _{t_{i_L}\to r_{i_L}}\circ E_{i_L})$} morphisms from their respective time semifields as developed for semileptons.
\vskip 11pt

So, the space-time internal vacuum of a \rl semibaryon is given by:
\begin{align*}
\wt M^{(\rm Bar);T_p-S_p}_{ST_R} &=\wt M^{(\rm Bar);T_p}_{ST_R}\bigoplus_{i=1}^3
\wt M^{q_i;T_p-S_p}_{ST_R}\\
\rresp{
\wt M^{(\rm Bar);T_p-S_p}_{ST_L} &=\wt M^{(\rm Bar);T_p}_{ST_L}\bigoplus_{i=1}^3
\wt M^{q_i;T_p-S_p}_{ST_L}}.\end{align*}
{\bf The} (operator-valued) {\bbf space-time string field
$(\wt M^{(\rm Bar);T_p-S_p}_{ST_R}\otimes \wt M^{(\rm Bar);T_p-S_p}_{ST_L})$ then describes the dynamics of the internal vacuum structure of a baryon %of the first family 
and corresponds to the dark energy structure of this baryon\/}.

It decomposes according to:
\begin{multline*}
(\wt M^{(\rm Bar);T_p-S_p}_{ST_R}\otimes \wt M^{(\rm Bar);T_p-S_p}_{ST_L})
=(\wt M^{(\rm Bar);T_p(r)}_{ST_R}\otimes \wt M^{(\rm Bar);T_p(r)}_{ST_L})\\
\bigoplus_{i=1}^3(\wt M^{q_i;T_p-S_p}_{ST_R}\otimes \wt M^{q_i;T_p-S_p}_{ST_L})
\bigoplus_{\substack{i=j=1\\ i\neq j}}^3(\wt M^{q_i;T_p-S_p}_{ST_R}\otimes \wt M^{q_j;T_p-S_p}_{ST_L})\\
\bigoplus_{i=1}^3(\wt M^{(\rm Bar);T_p(r)}_{ST_R}\otimes \wt M^{q_i;T_p-S_p}_{ST_L})
\bigoplus_{i=1}^3(\wt M^{q_i;T_p-S_p}_{ST_R}\otimes \wt M^{(\rm Bar);T_p(r)}_{ST_L})
\end{multline*}
where:
\Bi
\item $(\wt M^{(\rm Bar);T_p(r)}_{ST_R}\otimes \wt M^{(\rm Bar);T_p(r)}_{ST_L})$ is the core central time string field of the baryon, i.e. its {\bbf core dark energy structure\/};

\item $(\wt M^{q_i;T_p-S_p}_{ST_R}\otimes \wt M^{q_i;T_p-S_p}_{ST_L})$ is the internal vacuum string field of the $i$-th quark, i.e. {\bbf the dark energy structure of this quark\/}.  It decomposes into diagonal space and time string fields, magnetic and electric fields as envisaged before for the lepton;

\item $(\wt M^{q_i;T_p-S_p}_{ST_R}\otimes \wt M^{q_j;T_p-S_p}_{ST_L})$ are the mixed fields of interaction between the $i$-th right semiquark and the $j$-th left semiquark.  They decompose similarly into diagonal time and space fields of interaction, which are of gravitational nature as described in \cite{Pie7}, and into off diagonal magnetic and electric fields of interaction.  {\bbf These gravitational, electric and magnetic fields are ``dark energy interaction fields'' between quarks confined inside a baryon\/};

\item {\bbf $(\wt M^{(\rm Bar);T_p(r)}_{ST_R}\otimes \wt M^{q_i;T_p-S_p}_{ST_L})
\oplus(\wt M^{q_i;T_p-S_p}_{ST_R}\otimes \wt M^{(\rm Bar);T_p(r)}_{ST_L})$ are mixed  ``strong'' string fields of interaction between core central time string semifields of semibaryons and space-time string semifields of semiquarks.  They are responsible for the generation of ``meson dark energy''\/} after compactification of these interacting fields as developed in \cite{Pie8}.
\Ei
\vskip 11pt

\subsection{Bisemiparticle dark energy structure}

{\bbf The dark energy structure of an elementary particle then refers to the space-time fields of its internal vacuum structure, called space-time (ST)\/}.

As these fields are bisemifields,  i.e. products of right semifields by their symmetric left correspondents, an elementary particle at this dark energy level is a bisemiparticle composed of the product of a left semiparticle, localized in the upper half space, by its symmetric right (co)semiparticle, localized in the lower half space in such a way that:
\Bi
\item the space-time fields of its internal vacuum lead to a working interaction bisemispace responsible for the electric charge (i.e. the electric internal field), the magnetic moment (i.e. the magnetic internal space field), and an internal gravitational field in the case of a baryon;

\item the right semiparticle, dual of the left semiparticle, is projected on the latter and is unobservable unless the bisemiparticle be split into a pair of ``particle-antiparticle'' at this dark energy level.
\Ei

The leptons are then called bisemileptons and the baryons bisemibaryons.

Note that the bisemifermions of the second and third families have similar but much more complex structures than those of the first family.  They are generated from bisemifermions of the first family as described in \cite{Pie1} and in \cite{Pie8}.
\vskip 11pt

\subsection{Proposition}

{\bbf \em The dark energy structure of an elementary particle is a universal mathematical structure\/}.
\vskip 11pt

\begin{proof}
Indeed, the dark energy structure of an elementary particle is composed of the direct sum of a time field and of a space field localized in orthogonal (bisemi)spaces, or orthogonal to each other.  

On the other hand, each time or space dark energy string field is a bisemisheaf of rings as developed in proposition 2.4.

This bisemisheaf of rings is the analytic representation of the corresponding algebraic bilinear semigroup which is the representation of the product, right by left, of global Weil groups in the frame of the global program of Langlands as proved in \cite{Pie4} and recalled in section 2.3.

In the same context, this bisemisheaf gives rise to the product, right by left, of holomorphic functions (and/or cuspidal forms) by taking into account their power series development as developed in \cite{Pie3}.

Thus, the dark energy structure of an elementary particle, originating from algebraic biquanta generated by the product, right by left, of global Weil (or Galois) groups, can be represented by the sum of a time and a space holomorphic bifunction (and/or cuspidal biform).

This explains the universal mathematical character of the given dark energy structure of an elementary particle.
\end{proof}
%\vskip 11pt

\subsection{Does the dark energy of elementary particles correspond to a new kind of aether?}

The dark energy structure of elementary particles, being of space-time nature, is expansive since it is not confined by an external boundary shell. On the other hand, as this dark energy corresponds to the internal and generative primary structure of elementary particles, it fills uniformly the ``empty space''.

Thus, this dark energy may correspond to the aether \cite{Kra} of the physicists of the nineteenth century! \dots\ leading to a paradox since the aether wind was ruled out by the Michelson-Morley experiment.   This was the starting point of the special relativity of Einstein who postulated the invariance of the light velocity in the vacuum.

What is the solution of this apparent paradox?

The aether envisaged by the physicists of the nineteenth century was supposed to correspond to ``visible'' matter (the only defined matter at that time) which is composed, in the present context of algebraic quantum theory, of three embedded structure shells $\ST\subset \MG\subset \M$ ($\ST=$ space-time, $\MG=$ middle ground, $M=$ mass) defining the structure of (visible) massive elementary particles as it will be seen in the following chapter.  This is also the case of the light of which photons have a structure in three embedded shells 
$\ST\subset \MG\subset \M$.

Now, the dark energy, viewed as an aether, has an elementary particle composition made only of the ``$\ST$'' substructure.  Consequently, the only relevant interaction between the visible light and the ``dark energy aether'' seems to be at first sight between the ``$\ST$'' level of the dark energy and the boundary exterior shell ``$\M$'' of the visible light as it will be discussed in chapter 4.

But, as the rotational velocities, i.e. the frequencies of the shells ``$\ST$'' and ``$\M$'' are very different, no real quanta of interaction between these two shells can be effectively exchanged and thus, no real interaction exists between these two shells.

On the other hand, interactions still exist between the ``$\ST$'' structure of the dark energy and the ``$\ST$'' substructure of the light.  But, as the ``$\ST$'' vacuum substructure of the light is bounded by the ``$\MG$'' and ``$\M$'' exterior shells, no real quanta can be added to this one in order to increase its frequency.

Thus, it can be said that the dark energy could be interpreted as a new kind of aether differing from the aether of the nineteenth century physicists by the facts that:
\Bean
\item the dark energy does not really affect the velocity of the visible light;
\item the dark energy envisaged as an aether is not an absolute reference system.
\Ee


==> GL2_4.tex <==
\section{The dark energy and the dark matter structures of elementary particles interacting with the visible matter structure of other elementary particles}

\subsection{Bilinear interactions (dark energy case of bisemifermions)}

Let $(\wt M_{\ST_R}^{T_p-S_p}\otimes\wt M_{\ST_L}^{T_p-S_p})$,
$(\wt M_{\ST_R-\MG_R}^{T_p-S_p}\otimes\wt M_{\ST_L-MG_L}^{T_p-S_p})$ and
$(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}\otimes\wt M_{\ST_L-MG_L-\M_R}^{T_p-S_p})$
denote respectively the dark energy, dark matter and visible matter structures of an elementary bisemifermion (see section 3.1), the notation ``$\MG$'' replacing here the notation ``$\DM$''.
\vskip 11pt


Let $(\wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L}^{T_p-S_p}(I))$ denote
{\bbf the dark energy structure of ``$I$'' interacting elementary bisemifermions} on this unique level.  It {\bbf is the completely reducible nonorthogonal functional representation space of the bilinear algebraic semigroup}
$\GL_{2I}(L_{\o v}\times L_v)_{\ST}^{T_p-S_p}$ \cite{Pie6}:
\[
\L(\wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L}^{T_p-S_p}(I)\R)
= \FREPsp ( \GL_{2I}(L_{\o v}\times L_v))_{\ST}^{T_p-S_p}\;.\]
{\bbf Its time part} $\FREPsp ( \GL_{2I}(L_{\o v}\times L_v))_{\ST}^{T_p}$ {\bbf can be expressed as the cross binary product ``$\u\times$'' of its ``$I$'' bielements} according to \cite{Pie4}, \cite{Pie7}:
\begin{multline*}
\FREPsp ( \GL_{2I}(L_{\o v}\times L_v))_{\ST}^{T_p}\\
\begin{aligned}
 &= \FREPsp ( \GL_{2_1}(L_{\o v}\times L_v))_{\ST}^{T_p}\u\times \dots
\\
 & \qquad \u\times \FREPsp ( \GL_{2_i}(L_{\o v}\times L_v))_{\ST}^{T_p}\u\times \dots
\\
 & \qquad \qquad \u\times \FREPsp ( \GL_{2_I}(L_{\o v}\times L_v))_{\ST}^{T_p-S_p}\\
 %%
 &= \L(\bigoplus_{i=1}^I \FREPsp ( T^t_{2_i}(L_{\o v})_{\ST}^{T_p})\R)\times
  \L(\bigoplus_{i'=1}^I \FREPsp ( T^t_{2_{i'}}(L_{v})_{\ST}^{T_p})\R)\\
  %%
  &= \bigoplus_{i=1}^I \FREPsp ( \GL_{2_i}(L_{\o v}\times L_v))_{\ST}^{T_p}
\bigoplus_{i\neq i'=1}^I \FREPsp ( T^t_{2_i}(L_{\o v})\times T_{2_{i'}}(L_v))_{\ST}^{T_p}\\
%%
&\equiv \bigoplus_{i=1}^I(\wt M_{\ST_R}^{T_p}(i)\otimes\wt M_{\ST_L}^{T_p}(i))
\bigoplus_{i\neq i'=1}^I(\wt M_{\ST_R}^{T_p}(i)\otimes\wt M_{\ST_L}^{T_p}(i'))
\end{aligned}
\end{multline*}
{\bbf splitting
$(\wt M_{\ST_R}^{T_p}(I)\otimes\wt M_{\ST_L}^{T_p}(I))$ into ``$I$'' free time fields
$\{ (\wt M_{\ST_R}^{T_p}(i)\otimes\wt M_{\ST_L}^{T_p}(i))\}_{i=1}^I$ of
``$I$'' bisemifermions and into $(I^2-I)$ interacting time semifields
$\{ (\wt M_{\ST_R}^{T_p}(i)\otimes\wt M_{\ST_L}^{T_p}(i'))\}_{i\neq i'=1}^I$}
of the right and left semifermions belonging to different bisemifermions.
\vskip 11pt

\subsection{Proposition (Dark energy structure of $I$ bisemifermions)}

{\em {\bbf The dark energy structure of ``$I$'' interacting elementary bisemifermions is given by:}
\[%begin{multline*}
(\wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L}^{T_p-S_p}(I))%\\
= \bigoplus_{i=1}^I\L(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\ST_L}^{T_p-S_p}(i)\R)
\bigoplus_{i\neq i'=1}^I\L(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\ST_L}^{T_p-S_p}(i')\R)
\]%end{multline*}
where:
\Bean
\item {\bbf each free space-time field
$(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\ST_L}^{T_p-S_p}(i))$ of the dark energy structure } of an elementary bisemifermion {\bbf decomposes into a four-dimensional bilinear diagonal subfield, a three-dimensional off-diagonal magnetic subfield and into a three-dimensional off-diagonal electric subfield\/};

\item {\bbf each product, right by left, of space-time interacting semifields
$(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\ST_L}^{T_p-S_p}(i'))$} of the right and left dark energy semistructures of the interacting bisemifer\-mions $i$ and $i'$ {\bbf decomposes into a four-dimensional bilinear diagonal gravitational field, a three-dimensional interacting magnetic subfield and into a three-dimensional interacting electric subfield\/}.
\Ee
}
\vskip 11pt

\begin{proof}
\Be
\item The space dark energy structure of $I$ interacting bisemifermions can be handled similarly as it has been done for their time part in section 4.1 taking into account the morphism 
$(\gamma _{t\to r}\circ E_R)\times (\gamma _{t\to r}\circ E_L)$ transforming the time dark energy structure into its complementary space dark energy structure as developed in section 2.5.

\item The decomposition of the space-time internal fields
$(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\ST_L}^{T_p-S_p}(i))$
of an elementary bisemifermion ``$i$'' into diagonal, magnetic and electric subfields has been recalled in section 2.5.

\item The product, right by left, of the space-time interacting semifields $i$ and $i'$ decomposes similarly according to:
\begin{multline*}
(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\ST_L}^{T_p-S_p}(i'))
= (\wt M_{\ST_R}^{T_p-S_p}(i)\otimes_D\wt M_{\ST_L}^{T_p-S_p}(i'))\\
\oplus(\wt M_{\ST_R}^{S_p}(i)\otimes_{\rm magn}\wt M_{\ST_L}^{S_p}(i'))
\oplus(\wt M_{\ST_R}^{S_p(T_p)}(i)\otimes_{\rm elec}\wt M_{\ST_L}^{T_p(S_p)}(i'))
\end{multline*}
where:
\Bi
\item $(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes_D\wt M_{\ST_L}^{T_p-S_p}(i'))$ is a space-time gravitational field between the dark energy structures of the $i$-th right semifermion and the $i'$-th left semifermion as justified in \cite{Pie1}.  This gravitational field is generated by the exchange of (mixed) orthogonal gravitational biquanta;

\item $(\wt M_{\ST_R}^{S_p}(i)\otimes_{\rm magn}\wt M_{\ST_L}^{S_p}(i'))$ is a spatial magnetic field between the dark energy structures of the $i$-th right semifermion and the $i'$-th left semifermion.  This magnetic field is generated by the exchange of off-diagonal spatial magnetic biquanta.

\item $(\wt M_{\ST_R}^{S_p(T_p)}(i)\otimes_{\rm elec}\wt M_{\ST_L}^{T_p(S_p)}(i'))$ is a space-time (or time-space) electric field generated by the exchange of space-time (or time-space) electric biquanta between the dark energy structures of the $i$-th right semifermion and the $i'$-th left semifermion.\qedhere
\Ei
\Ee
\end{proof}
\vskip 11pt

\subsection{Proposition (Dark mass structure of $J$ (interacting) bisemifermions)}

{\em
{\bbf The dark mas structure of ``$J$'' interacting elementary bisemifermions is given by:}
\begin{multline*}
(\wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\otimes\wt M_{\ST_L-\MG_L}^{T_p-S_p}(J))\\
\begin{aligned}
&=(\wt M_{\ST_R}^{T_p-S_p}(J)\oplus\wt M_{\MG_R}^{T_p-S_p}(J))\otimes(\wt M_{\ST_L}^{T_p-S_p}(J)\oplus\wt M_{\MG_L}^{T_p-S_p}(J))\\
%%
&=\L\{ \L[ 
\bigoplus_{j=1}^J(\wt M_{\ST_R}^{T_p-S_p}(j)\otimes\wt M_{\ST_L}^{T_p-S_p}(j))
\bigoplus_{j=1}^J(\wt M_{\MG_R}^{T_p-S_p}(j)\otimes\wt M_{\MG_L}^{T_p-S_p}(j))
\R] \R.\\
%%
&\quad \L.\L[
\bigoplus_{j=1}^J (\wt M_{\ST_R}^{T_p-S_p}(j)\otimes\wt M_{\MG_L}^{T_p-S_p}(j))
\bigoplus_{j=1}^J (\wt M_{\MG_R}^{T_p-S_p}(j)\otimes\wt M_{\ST_L}^{T_p-S_p}(j))
\R] \R\}\\
%%
&\qquad \L\{ \L[
\bigoplus_{j\neq j'=1}^J (\wt M_{\ST_R}^{T_p-S_p}(j)\otimes\wt M_{\ST_L}^{T_p-S_p}(j'))
\bigoplus_{j\neq j' =1}^J (\wt M_{\MG_R}^{T_p-S_p}(j)\otimes\wt M_{\MG_L}^{T_p-S_p}(j'))\R]\R.\\
%%
&\quad\qquad \L.\L[
\bigoplus_{j\neq j'=1}^J (\wt M_{\ST_R}^{T_p-S_p}(j)\otimes\wt M_{\MG_L}^{T_p-S_p}(j'))
\bigoplus_{j\neq j'=1}^J (\wt M_{\MG_R}^{T_p-S_p}(j)\otimes\wt M_{\ST_L}^{T_p-S_p}(j'))
\R] \R\}\end{aligned}\end{multline*}
{\bbf where:}
\Bean
\item {\bbf the direct sum of fields inside the first parenthesis $\{\cdot\}$ refers to the internal structure fields ``$\ST$'' and ``$\MG$'' of the $J$ free dark massive bisemifermions as well as to the interacting internal electro-magnetic fields} between the right ``$\ST$''  \resp{right ``$\MG$''} semistructures and the left ``$\MG$'' \resp{left ``$\ST$''} semistructures of these free dark massive bisemifermions;

\item {\bbf the direct sum of interacting bilinear fields inside the second parenthesis $\{\cdot\}$ refers to the gravito-electro-magnetic fields\/} between the ``$\ST$''  and ``$\MG$'' right and left shells belonging to different bisemifermions as well as the gravito-electro-magnetic fields between mixed right and left ``$\ST$''  and ``$\MG$'' shells belonging to different bisemifermions.
\Ee
}
\vskip 11pt

\begin{proof}
\Bean
\item The dark mass structure of $J$ interacting elementary bisemifermions
$(\wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\linebreak \otimes\wt M_{\ST_L-\MG_L}^{T_p-S_p}(J))$ is given by the tensor product of right and left direct sums of their space-time
``$\ST$'' and middle-ground ``$\MG$'' semistructures on the consideration that it is a completely reducible non-orthogonal functional representation space of the mixed bilinear algebraic semigroup
$\GL_{2J}(L_{\o v}\times L_v)_{\ST+\MG}^{T_p-S_p}$ according to section 4.1.

\item Let us analyze the different fields responsible for the dark mass structure of these interacting bisemifermions
\Be
\item $\bigoplus_{j=1}^J(\wt M_{\ST_R}^{T_p-S_p}(j)\otimes\wt M_{\ST_L}^{T_p-S_p}(j))$ and
$\bigoplus_{j=1}^J(\wt M_{\MG_R}^{T_p-S_p}(j)\otimes\wt M_{\MG_L}^{T_p-S_p}(j))$ are respectively the ``$\ST$''  and ``$\MG$'' internal fields of these $J$ bisemifermions decomposing into diagonal, magnetic and electric subfields as envisaged in proposition 4.2.

\item $\bigoplus_{j=1}^J (\wt M_{\ST_R}^{T_p-S_p}(j)\otimes\wt M_{\MG_L}^{T_p-S_p}(j))$ and
$\bigoplus_{j=1}^J (\wt M_{\MG_R}^{T_p-S_p}(j)\otimes\wt M_{\ST_L}^{T_p-S_p}(j))$ are respectively mixed interaction semifields between the right ``$\ST$''-left ``$\MG$'' and the right
``$\MG$''--left ``$\ST$'' semistructures of these free bisemifermions.

These gravito-electro-magnetic interacting fields between mixed subsemistructures are likely not very relevant because the frequencies of the ``$\ST$''  and ``$\MG$'' shells are not of the same order preventing the exchange of biquanta.

\item $\bigoplus_{j\neq j'=1}^J (\wt M_{\ST_R}^{T_p-S_p}(j)\otimes\wt M_{\ST_L}^{T_p-S_p}(j'))$ and
$\bigoplus_{j\neq j'=1}^J (\wt M_{\MG_R}^{T_p-S_p}(j)\otimes\wt M_{\MG_L}^{T_p-S_p}(j'))$ are respectively interaction fields between the 
``$\ST$''  and ``$\MG$'' right and left semistructures belonging to different bisemifermions.

They decompose usually respectively into ``$\ST$''  and ``$\MG$'' gravito-electro-magnetic fields.

\item $\bigoplus_{j\neq j'=1}^J (\wt M_{\ST_R}^{T_p-S_p}(j)\otimes\wt M_{\MG_L}^{T_p-S_p}(j'))$ and
$\bigoplus_{j\neq j'=1}^J (\wt M_{\MG_R}^{T_p-S_p}(j)\otimes\wt M_{\ST_L}^{T_p-S_p}(j'))$ are respectively mixed ``$\ST_R-\MG_L$'' and
``$\MG_R-\ST_L$'' interaction fields between different right and left semifermions.

Their decomposition into GEM (gravito-electro-magnetic) fields does not probably give rise to an effective exchange of biquanta.\qedhere
\Ee
\Ee
\end{proof}
\vskip 11pt

\subsection{Proposition (Visible mass structure of $K$ (interacting) bisemifermions)}

{\em
{\bbf The visible mass structure of ``$K$'' interacting elementary bisemifermions is given by\/}:
\begin{multline*}
(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))\\
\begin{aligned}
&=(\wt M_{\ST_R}^{T_p-S_p}(K)\oplus\wt M_{\MG_R}^{T_p-S_p}(K)\oplus\wt M_{\M_R}^{T_p-S_p}(K))\otimes
(\wt M_{\ST_L}^{T_p-S_p}(K)\oplus\wt M_{\MG_L}^{T_p-S_p}(K)\oplus\wt M_{\M_L}^{T_p-S_p}(K))\\
%%
&=\L\{ \L[ 
\bigoplus_{k=1}^K(\wt M_{\ST_R}^{T_p-S_p}(k)\otimes\wt M_{\ST_L}^{T_p-S_p}(k))
\bigoplus_{k=1}^K(\wt M_{\MG_R}^{T_p-S_p}(k)\otimes\wt M_{\MG_L}^{T_p-S_p}(k))
\bigoplus_{k=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k))
\R] \R.\\
%%
& \qquad \L[
\bigoplus_{k=1}^K(\wt M_{\ST_R}^{T_p-S_p}(k)\otimes\wt M_{\MG_L}^{T_p-S_p}(k))
\bigoplus_{k=1}^K(\wt M_{\MG_R}^{T_p-S_p}(k)\otimes\wt M_{\ST_L}^{T_p-S_p}(k))
\bigoplus_{k=1}^K(\wt M_{\ST_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k))\R.
\\
%%
& \qquad \L. \L.
\bigoplus_{k=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\ST_L}^{T_p-S_p}(k))
\bigoplus_{k=1}^K(\wt M_{\MG_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k))
\bigoplus_{k=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\MG_L}^{T_p-S_p}(k))
\R] \R\}\\
%%
& \qquad \quad \L\{ \L[ 
\bigoplus_{k\neq k'=1}^K(\wt M_{\ST_R}^{T_p-S_p}(k)\otimes\wt M_{\ST_L}^{T_p-S_p}(k'))\R.\R.
\begin{aligned}[t]
&\bigoplus_{k\neq k'=1}^K(\wt M_{\MG_R}^{T_p-S_p}(k)\otimes\wt M_{\MG_L}^{T_p-S_p}(k'))\\
%
&  \qquad \L.
\bigoplus_{k\neq k'=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k'))\R]
\end{aligned}\\
%%
& \qquad \qquad  \L[ 
\bigoplus_{k\neq k'=1}^K(\wt M_{\ST_R}^{T_p-S_p}(k)\otimes\wt M_{\MG_L}^{T_p-S_p}(k'))\R.
\begin{aligned}[t]
&\oplus \dots \oplus
\bigoplus_{k\neq k'=1}^K(\wt M_{\ST_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k'))\\
& \quad \L.\L.\oplus \dots\oplus
\bigoplus_{k\neq k'=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\MG_L}^{T_p-S_p}(k'))\R]\R\}
\end{aligned}
\end{aligned}
\end{multline*}
where:
\Bean
\item the direct sum of fields inside the first parenthesis $\{\cdot\}$ refers to the internal structure fields ``$\ST$'', ``$\MG$'' and ``$\M$'' of the ``$K$'' free (visible) massive bisemifermions as well as to the interacting internal mixed electro-magnetic fields between the right ``$\ST$'', ``$\MG$'' and ``$\M$'' semistructures of these free massive bisemifermions and their corresponding left mixed equivalents;

\item the direct sum of interacting bilinear fields inside the second parenthesis $\{\cdot\}$ refers to the gravito-electro-magnetic fields between the ``$\ST$'', ``$\MG$'' and ``$\M$'' right and left shells belonging to different bisemifermions as well as to the GEM fields between mixed right and left ``$\ST$'', ``$\MG$'' and ``$\M$'' shells of these.
\Ee
}
\vskip 11pt

\begin{proof}
The visible mass structure of interacting bisemifermions corresponds to their dark mass structure to which the ``$\M$'' fields
$(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k))$ have been added.

Thus, the different fields responsible for this visible mass structure are those of the corresponding (i.e. at ``$K$'' interacting massive bisemifermions) dark mass structure plus:
\Bena
\item $\bigoplus_{k=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k))$ which are the ``$\M$'' internal fields of the $K$ bisemifermions decomposing into diagonal, magnetic and electric subfields;

\item the mixed interaction semifields
$\bigoplus_{k=1}^K(\wt M_{\ST_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k))
\bigoplus_{k=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\ST_L}^{T_p-S_p}(k))\linebreak
\bigoplus_{k=1}^K(\wt M_{\MG_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k))
\bigoplus_{k=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\MG_L}^{T_p-S_p}(k))$ between the right ``$\ST$'' and ``$\MG$''--left ``$\M$'' and the right ``$\M$''--left ``$\ST$'' and ``$\MG$'' semistructures of these free bisemifermions;

\item the interactions fields
$\bigoplus_{k\neq k'=1}^K(\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k'))$ between the ``$\M$'' right and left semistructures belonging to different bisemifermions;

\item the mixed 
``$\ST_R-\M_L$'',
``$\M_R-\ST_L$'',
``$\MG_R-\M_L$'' and
``$\M_R-\MG_L$'' interaction semifields
$\L(\bigoplus_{k\neq k'=1}^K\wt M_{\ST_R}^{T_p-S_p}(k)\otimes\wt M_{\M_L}^{T_p-S_p}(k')\R)\ \dots\ 
\L(\bigoplus_{k\neq k'=1}^K\wt M_{\M_R}^{T_p-S_p}(k)\otimes\wt M_{\MG_L}^{T_p-S_p}(k')\R)$ between different left and right semifermions.\qedhere
\Ee
\end{proof}
\vskip 11pt

\subsection{Proposition (Interaction between ``$I$'' dark energetic bisemifermions and ``$K$'' visible massive bisemifermions)}

{\em
{\bbf The interactions between ``$I$'' dark energetic bisemifemions and ``$K$'' visible massive bisemifermions decompose into:
\Bean
\item ``$I$'' interacting dark energetic (elementary) bisemifermions and ``$K$'' interacting visible massive (elementary) bisemifermions;

\item plus the GEM interaction fields between the \rl dark energy semistructures of the ``$I$'' \rl semifermions and the \lr ``$\ST$'', ``$\MG$'' and ``$\M$'' subsemistructures of the ``$K$'' visible semi\-fermions.
\Ee
}}
\vskip 11pt

\begin{proof}
The interaction between the dark energy structure
$(\wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L}^{T_p-S_p}(I))$ of $I$ elementary bisemifermions and the visible mass structure
$(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes \wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))$ of $K$ different elementary bisemifermions is described by:
\begin{multline*}
(\wt M_{\ST_R}^{T_p-S_p}(I)\oplus\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes
(\wt M_{\ST_L}^{T_p-S_p}(I)\oplus\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))\\
%
= \L[ \L( \wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L}^{T_p-S_p}(I)\R)\oplus
\L(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K) \R) \R]\\
%%
\oplus\L[ \L( \wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K)\R)\oplus
 \L( \wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes
\wt M_{\ST_L}^{T_p-S_p}(I) \R) \R]
\end{multline*}
where:
\Bean
\item {\bbf the set of fields $(\wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L}^{T_p-S_p}(I))$ and
$(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes\linebreak \wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))$ refers respectively to the dark energy structure of ``$I$'' interacting elementary bisemifermions} as described in proposition 4.2 {\bbf and to the visible mass structure of $K$ interacting elementary bisemifemions} as described in proposition 4.4;

\item {\bbf the set of fields
$(\wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))$
\resp{$(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes\linebreak \wt M_{\ST_L}^{T_p-S_p}(I))$} 
refers to the interacting fields between the right dark energy semistructures} \resp{right visible mass semistructures} {\bbf of the ``$I$'' right semifermions} \resp{the ``$K$'' right semifermions} {\bbf and the left visible mass semistructures} \resp{the left dark energy semistructures} {\bbf of the  ``$K$'' left semifermions} \resp{the ``$I$'' left semifermions}.
\Ee

We shall only focus on the fields of interaction
$(\wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))$ between right dark energy semistructures and left visible mass semistructures, the fields $(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes \wt M_{\ST_L}^{T_p-S_p}(I))$ being strictly symmetric to the firsts.

They develop according to:
\begin{multline*}
(\wt M_{\ST_R}^{T_p-S_p}(I)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))\\
\begin{aligned}
& =\L[ 
\L( 
\bigoplus _{i=1}^I\wt M_{\ST_R}^{T_p-S_p}(i)
\R)
\otimes
 \L( 
\bigoplus _{k=1}^K\wt M_{\ST_L}^{T_p-S_p}(k)
 \bigoplus _{k=1}^K\wt M_{\MG_L}^{T_p-S_p}(k)
 \bigoplus _{k=1}^K\wt M_{\M_L}^{T_p-S_p}(k)
\R)
\R]\\
 %%
 & =
\L[ 
\L( 
\L( 
\bigoplus _{i=1}^I\wt M_{\ST_R}^{T_p-S_p}(i)\R)\otimes
 \L( \bigoplus _{k=1}^K\wt M_{\ST_L}^{T_p-S_p}(k)\R)\R)\R.
 \begin{aligned}[t]
 &\oplus
 \L( \L(\bigoplus _{i=1}^I\wt M_{\ST_R}^{T_p-S_p}(i)\R)\otimes
 \L(\bigoplus _{k=1}^K\wt M_{\MG_L}^{T_p-S_p}(k)\R)\R)\\
 %%
 &\qquad \oplus
 \L.\L(\L( \bigoplus _{i=1}^I\wt M_{\ST_R}^{T_p-S_p}(i)\R)\otimes
 \L(\bigoplus _{k=1}^K\wt M_{\M_L}^{T_p-S_p}(k)\R)\R)\R]
 \end{aligned}
 \end{aligned}
 \end{multline*}
 where:
 \Bean
 \item $( \bigoplus _{i=1}^I\wt M_{\ST_R}^{T_p-S_p}(i))\otimes
 ( \bigoplus _{k=1}^K\wt M_{\ST_L}^{T_p-S_p}(k))$ are fields of interaction between the right dark energy semistructures of the ``$I$'' right semifermions and the left ``$\ST$'' subsemistructures of the ``$K$'' left semifermions.
 
 The $(i-k)$-th interaction fields
$(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\ST_L}^{T_p-S_p}(k))$ decomposes into GEM (gravito-electro-magnetic) fields at this ``$\ST$'' level as developed in proposition 4.2.

\item Similarly, the  $(i-k)$-th interaction fields
$(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\MG_L}^{T_p-S_p}(k))$ and
$(\wt M_{\ST_R}^{T_p-S_p}(i)\otimes\wt M_{\M_L}^{T_p-S_p}(k))$  between the right dark energy semistructure of the $i$-th right semifermion and, respectively, the left ``$\MG$'' and ``$\M$'' subsemistructures of the $k$-th left visible massive semifermion 
decomposes into GEM  fields at these ``$\MG$'' and ``$\M$'' levels as noticed in proposition 4.4.  It is likely that these interaction fields are not very important as previously noted.\qedhere
\Ee
\end{proof}
\vskip 11pt

\subsection{Proposition (Interaction between ``$J$'' dark massive bisemifermions and ``$K$'' visible massive bisemifermions)}

{\em
{\bbf The interaction between ``$J$'' dark massive bisemifermions and ``$K$'' visible massive bisemifermions decomposes into:
\Bean
\item ``$J$'' interacting dark massive bisemifermions and ``$K$'' interacting visible massive bisemifermions;

\item plus the GEM interaction fields between the \rl dark massive semistructures of the ``$J$'' \rl semifermions and the \lr visible massive semistructures of the ``$K$'' \lr semifermions.
\Ee}}
\vskip 11pt

\begin{proof}
The interaction between the dark mass structure
$(\wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\otimes\wt M_{\ST_L-\MG_L}^{T_p-S_p}(J))$ of
``$J$'' elementary bisemifermions and the visible mass structure
$(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes\linebreak \wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))$ of ``$K$'' different elementary bisemifermions is given by:
\begin{multline*}
\L(\wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\oplus\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\R)
\otimes
\L(\wt M_{\ST_L-\MG_L}^{T_p-S_p}(J)\oplus\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K)\R)\\
= \L[
\L(\wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\otimes\wt M_{\ST_L-\MG_L}^{T_p-S_p}(J)\R)
\oplus
\L(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K)\R)\R]\\
%%
\oplus \L[
\L(\wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K)\R)
\oplus
\L(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes\wt M_{\ST_L-\MG_L}^{T_p-S_p}(J)\R)\R]
\end{multline*}
where:
\Bean
\item the set of fields in the first parenthesis $[(\cdot)\oplus(\cdot)]$ refers respectively to the dark mass structure of  ``$J$''  interacting elementary bisemifermions as described in proposition 4.3 and to the visible mass structure of ``$K$'' interacting elementary bisemifermions;

\item the set of fields in the second parenthesis
$(\wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))
$ and $
(\wt M_{\ST_R-\MG_R-\M_R}^{T_p-S_p}(K)\otimes\wt M_{\ST_L-\MG_L}^{T_p-S_p}(J))$
refers to the interaction fields between the right dark matter semistructures \resp{right visible matter semistructures} of the ``$J$'' right semifermions \resp{``$K$'' right semifermions} and  the left visible matter semistructures \resp{the left dark matter semistructures} of the ``$K$'' left semifermions \resp{the ``$J$'' left semifermions}.
\Ee

As in proposition 4.5, we shall only analyze the fields of interaction
$(\wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\otimes\linebreak \wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K))
$ between the right dark matter semistructures and the left visible matter semistructures.

They develop according to:
\begin{multline*}
\L( \wt M_{\ST_R-\MG_R}^{T_p-S_p}(J)\otimes\wt M_{\ST_L-\MG_L-\M_L}^{T_p-S_p}(K)\R)\\
\begin{aligned}
&= 
\L[ 
\L( 
\L(
\bigoplus_{j=1}^J\wt M_{\ST_R}^{T_p-S_p}(j)
\R) 
\otimes   
\L(
\bigoplus_{k=1}^K\wt M_{\ST_L}^{T_p-S_p}(k)
\R)
\R)
\oplus
\L(
\L(
\bigoplus_{j=1}^J\wt M_{\MG_R}^{T_p-S_p}(j)
\R) 
\otimes  
\L(
\bigoplus_{k=1}^K\wt M_{\MG_L}^{T_p-S_p}(k)
\R)
\R)
\R.\\
%%
& \quad \oplus
\L(
\L( 
\bigoplus_{j=1}^J\wt M_{\ST_R}^{T_p-S_p}(j)
\R) 
\otimes  
\L(
\bigoplus_{k=1}^K\wt M_{\MG_L}^{T_p-S_p}(k)
\R)
\R)
\oplus
 \L(
\L(
\bigoplus_{j=1}^J\wt M_{\MG_R}^{T_p-S_p}(j)
\R) 
\otimes  
\L( 
\bigoplus_{k=1}^K\wt M_{\ST_L}^{T_p-S_p}(k)
\R)
\R)   \\
%%
& \quad  \oplus 
\L.
\L(
\L(
\bigoplus_{j=1}^J\wt M_{\ST_R}^{T_p-S_p}(j) 
\R)
\otimes  
\L( 
\bigoplus_{k=1}^K\wt M_{\M_L}^{T_p-S_p}(k)\R)\R)\oplus
\L(\L(\bigoplus_{j=1}^J\wt M_{\MG_R}^{T_p-S_p}(j)\R)\R) \otimes \L(\L( \bigoplus_{k=1}^K\wt M_{\M_L}^{T_p-S_p}(k)\R)\R)\R]
\end{aligned}
\end{multline*}
where:
\Bean
\item $\L( \L(\bigoplus_{j=1}^J\wt M_{\ST_R}^{T_p-S_p}(j)\R) \otimes   \L(\bigoplus_{k=1}^K\wt M_{\ST_L}^{T_p-S_p}(k)\R)\R)$ and
$\L( \L(\bigoplus_{j=1}^J\wt M_{\MG_R}^{T_p-S_p}(j) \R)\otimes   \L(\bigoplus_{k=1}^K\wt M_{\MG_L}^{T_p-S_p}(k)\R)\R)$ are mixed GEM interaction fields 
between the ``$\ST$'' right and left semistructures
of the ``$J$'' right and ``$K$'' left semifermions and between the ``$\MG$'' right and left semistructures of the same set of semifermions;

\item the four other interaction fields are mixed GEM interaction fields between mixed right and left semistructures of the $J$ right and $K$ left semifermions.\qedhere
\Ee
\end{proof}
\vskip 11pt

\subsection{Remark}

This chapter has treated the interaction between sets of elementary bisemifermions, i.e. the (bisemi)leptons and the (bisemi)quarks, being visible massive, dark massive or dark energetic.

The extension of this treatment to (bisemi)baryons will not be envisaged here but can be handled easily by taking into account my preprint \cite{Pie8} and section 2.5.



